TNS: Terrain Traversability Mapping and Navigation System for Autonomous Excavators

We present a terrain traversability mapping and navigation system (TNS) for autonomous excavator applications in an unstructured environment. We use an efficient approach to extract terrain features from RGB images and 3D point clouds and incorporate them into a global map for planning and navigation. Our system can adapt to changing environments and update the terrain information in real-time. Moreover, we present a novel dataset, the Complex Worksite Terrain (CWT) dataset, which consists of RGB images from construction sites with seven categories based on navigability. Our novel algorithms improve the mapping accuracy over previous SOTA methods by 4.17-30.48% and reduce MSE on the traversability map by 13.8-71.4%. We have combined our mapping approach with planning and control modules in an autonomous excavator navigation system and observe 49.3% improvement in the overall success rate. Based on TNS, we demonstrate the first autonomous excavator that can navigate through unstructured environments consisting of deep pits, steep hills, rock piles, and other complex terrain features.

==> sections/4-perception_sol_execavator.tex <==
\section{Terrain Traversability Mapping}




In this section, we present an efficient 2D-3D hybrid method for terrain traversability mapping and navigation system (\ours{}) to extract terrain features and generate a traversability map as the robot navigates through an unknown environment. \ours{} takes a 3D point cloud stream from the LiDAR, an RGB camera stream from the RGB camera, and the corresponding poses of the excavator extracted from the GPS-RTK module. The output of our method is a global map consisting of terrain information, including semantic information, geometric information, and a final traversability score.




% Our method is a hybrid method that combines 2D semantic and 3D geometric information. Most of the existing methods~\cite{geo1,voxel_classification} use 3D point cloud or voxels to detect obstacles and classify them into different terrain types, while some methods like~\cite{semantic_mapping, semantic_only_cmp4} only use 2D semantic segmentation and register terrain labels on the point cloud. Combining both 2D semantic information and 3D geometric information is essential for a robust prediction. For example, we can use geometric information from point clouds to detect pits or hills, while it is difficult to get such terrain information from an RGB photo. On the other hand, 2D semantic segmentation can provide terrain semantics through visual features. For example, a terrain with a flat surface indicated through LiDAR detection could still be a water puddle, or a surface with a high slope could be a small pile of dirt, which is traversable, or a rock pile, which needs to be avoided. 

% There are some reasons why we choose not to use 3D segmentation methods directly on the point cloud. First, it is difficult to annotate 3D data with semantic labels, while 2D labels are more accessible and easier to annotate. Second, 3D segmentation networks are usually heavy models and require longer inference time. Finally, during navigation in unstructured environments, excavator tracks could cause dust in the air, which introduces a lot of noise for the LiDAR input. 2D RGB images have rich color and texture information and are more immune to dust.

%The rest of this section is structured as follows: We start with a problem definition and motivation of our task for terrain traversability mapping in unstructured terrain in Section~\ref{def}. Then, we discuss two components of our method: semantic mapping and geometric computation in Section~\ref{semantic} and Section~\ref{geometric}, respectively. We discuss how to use combined information to estimate terrain traversability in Section~\ref{trav_est}. 



\subsection{Perception for Outdoor Excavators}
\label{def}

% In this section, we gave some backgrounds on navigation problem for excavator in unstructured environment, and give a formal definition of the problem we try to solve. 

\begin{figure*}[t]
    \vspace{3pt}
    \centering
    \includegraphics[width=\textwidth]{fig/pipeline2.png}
    \caption{\textbf{Overview of our method (\ours{}):} Our method takes RGB images and point clouds as inputs to infer traversability. We extract semantic information using segmentation and associate terrain labels with point clouds, as shown in A (\textbf{top}). We extract geometric information using slope and step height estimation, as shown in B (\textbf{bottom}). Finally, we produce a traversability gridmap based on semantic and geometric information and convert it to a 2D occupancy map for path planning, as shown in C (\textbf{right}).}
    \label{fig:overview}
    \vspace{-18pt}
\end{figure*}

The road conditions in structured environments such as highways are usually navigation-friendly, so the core problem during navigation in structured environments is avoiding obstacles rather than determining which part of the surface is easier and safer to navigate. 
% The boundaries of different objects in structured, urban environments can be clearly captured by perception methods, which reduces the likelihood of mis-classifications. 
In contrast, excavators are usually operated in unstructured and dangerous environments consisting of rock piles, cliffs, deep pits, steep hills, etc. 
% An unstructured environment usually refers to a terrain that lacks structure and has unpredictable and potentially hazardous conditions. 
Such an environment lacks any lane markings, and the arrangement of obstacles tends to be non-uniform. 
In addition, due to tasks like digging and dumping, the working conditions for excavators are constantly changing. Landfalls and cave-ins occur, potentially causing the excavator to tip over and injure the operator. Therefore, it is crucial to identify different terrains and predict safe regions for navigation. 

The definition of traversability is, according to~\cite{survey1}, the capability of a ground vehicle to reside over a terrain region under an admissible state wherein it is capable of entering given its current state. In order to solve navigation challenges for excavators as well as other working vehicles in unstructured terrain, we formulate the problem of obtaining an accurate traversability map representation as follows:

\noindent\textbf{Problem Definition:} Given sensor inputs $S_1, S_2, .., S_h$ from $h$ different sources, over a time span $T$, the goal is to obtain a 2D grid map $T\in[0, 1]^{H \times W}$ with resolution $r$, where $T$ corresponds to some region $R$ of shape $(Hr, Wr)$. The maximum value 1 corresponds to a non-traversable region, while the minimum value 0 corresponds to the most traversable region.

\noindent\textbf{Metrics for Traversability Map:} We need to consider the following measurements in excavator applications:
% \vspace{-6pt}


\begin{itemize}
%   \setlength\itemsep{-0.5em}
    \item \textbf{Accuracy:} Similar to~\cite{2D3D, pc_desert_cmp1, 3d_cam_cmp3}, we use an ROC curve to measure the accuracy of the traversability prediction. In addition, the map output should fit the terrain closely, so we also use MSE (mean squared error) as a fitness measurement.
    \item \textbf{Performance:} \cite{semantic_only_cmp4, semantic_for_planning_cmp2} use navigation outcome to measure their terrain traversability mapping algorithms, which include travel time, success rate, etc.
    \item \textbf{Energy constraints and run-time:} Due to the limitations of hardware and power supply on the excavator, energy efficiency and run-time should also be measured in a terrain traversability mapping method.
\end{itemize}
% \vspace{-6pt}

\noindent\textbf{Our Solution -- \ours{}:} 
The map is represented as an elevation grid map and is updated based on incoming point clouds and RGB images.
Internally, each grid cell in the map stores the average height value of the latest $p$ points within this cell, as well as overall information about those points like update time, slope, step height, and their semantic information. A traversability score is calculated for each grid cell. In Figure~\ref{fig:overview}, we present an overview of our approach. Our code is based on the open-source gridmap library~\cite{fankhauser2016universal}.



% energy constrain



% State 

% add metrics 



% We explain how we process the output traversability map and integrate it with path planning and navigation in Section~\ref{navi}.
% Finally, we discuss how the terrain map was constructed and updated for each time step in Section~\ref{mapping}.


% \subsection{Semantic Information Fusion with Point Cloud}
\vspace{-5pt}
\subsection{Segmentation and Mapping to Point Cloud}
\label{semantic}

% \input{tables/classes}

We use 2D semantic segmentation on unstructured terrains. Given an input RGB image $I \in \mathbb{R}^{3\times H \times W}$,
% and the corresponding terrain labels $Y\in \mathbb{Z}^{H\times W}$,
the goal is to generate a mask $P\in\{0, 1, ..., N - 1\}^{H \times W}$, where $N$ is the number of classes. We use Fast-SCNN~\cite{fastscnn} after leveraging accuracy and efficiency, as shown in Table~\ref{tab:flops}.
% Based on previous analysis~\ref{dataset}, we choose \tian{XXX} as our segmentation model.

% To better facilitate the learning process, we create a novel Autonomous Exccavator Terrain (AET) dataset for terrain classification and obstacle detection.
% % Our training data is collected in a construction site. %in Xuzhou. 
% According to the traversability criterion of the navigable regions defined in latest work~\cite{guan2021ganav} and the operating environments of excavators, we define seven classes in AET dataset, including flat regions, bumpy regions, mixed water and dirt, water puddles, rock piles, obstacles, and other excavators. The goal of the annotation is to identify different traversable regions and obstacles during navigation. 
% % , we define traversable regions in our method and dataset as shown in table~\ref{tab:classes}.
%  Based on AET dataset, we train a Fast-SCNN~\cite{fastscnn} model for finding traversable regions with real-time performance. Our training code is based on \cite{mmseg2020}. For more details about AET dataset, please refer to Section~\ref{data}.

% After we get the segmentation prediction $P$, we use a timestamp to locate the corresponding point cloud $C$. Given a point $\vec{p} = [x_p, y_p, z_p]\in C$ in the world coordinate, camera intrinsic matrix $K \in\mathbb{R}^{3\times 3}$, and extrinsic matrix $E\in\mathbb{R}^{4\times 4}$, we can calculate its corresponding image coordinates $\vec{p_i} = [u, v]$ based on the following formula:
% $$
% \begin{pmatrix}
% x_c \\
% y_c \\
% z_c \\
% 1
% \end{pmatrix}
%  = 
%  E \cdot 
% \begin{pmatrix}
% x_p \\
% y_p \\
% z_p \\
% 1
% \end{pmatrix} \\
% % \begin{pmatrix}
% % u \\
% % v \\
% % 1
% % \end{pmatrix}
% %  = 
% %  K \cdot
% % \begin{pmatrix}
% % x_c \\
% % y_c \\
% % z_c
% % \end{pmatrix}
% %  / z_c
% $$

% $$
% \hspace{15pt}
% \begin{pmatrix}
% u \\
% v \\
% 1
% \end{pmatrix}
%  = 
%  K \cdot
% \begin{pmatrix}
% x_c \\
% y_c \\
% z_c
% \end{pmatrix}
%  / z_c
% $$

After we get the segmentation prediction $P$, we use a timestamp to locate the corresponding point cloud $C$ and use camera calibration matrices to find the correspondence of each point to the segmentation results and save the terrain label in the gridmap cell. 
% In the end, each gridmap cell is assigned a terrain label based on the majority rule. 
% of the semantic labels. 
% For cells that are not assigned with a semantic label, we extract geometric information as a replacement for traversability estimation.



\subsection{Geometric Information Computation}
\label{geometric}

In this section, we present details of slope and step height estimation and highlight how machine specifications are considered to calculate geometric traversability score.
% Based on the height value in each grid map cell, we extract geometric information, including slope and step height, and use that as indications of terrain traversability. 
% Different from \cite{geo1}, we exclude the calculation of roughness in our formulation since excavators are designed to handle relatively rough terrains. In addition, roughness can be partially described either through slope and step height, or be captured by visual features from the RGB images. 
% In addition, our experiments and data are based on real-world scenarios in a construction site. 
% Our method also adapts to the physical constraints of excavators to determine threshold, resolution of the grid and $k$ neighbors.
% In addition, all of the estimations are parameterized by size, weight \tian{and xxx} of the vehicle to adapt to different scenarios and machines.
% Explain here how to we leverate physical property of the robot
% How to denoise? 

\noindent\textbf{Slope Estimation:} Each grid cell $g$ is abstracted to a single point $p = \{x, y, z\}$, where $x$, $y$ is the center of the cell in the global coordinate frame and $z$ is the height value of the grid.
The slope $s$ in arbitrary grid cell $g$ is computed by the angle between the surface normal and the z-axis\footnote{Up direction in the real world} of the global coordinate frame:
$$
s = arcos({n}^z), {n}^z \in [0, 1]
$$
where ${n}^z$ is the component of normal $\vec{n}$ on the z-axis.


We use Principal Component Analysis (PCA) to calculate the normal direction of a grid cell. The covariance matrix $C_{cov}$ of the nearest neighbors of the query grid cell is calculated as follows:
\vspace{-3pt}
$$
C_{cov} = \frac{1}{k} \sum_{i=1}^{k} (p_i - \bar{p}) \cdot (p_i - \bar{p})^T , \ C_{cov} \cdot \vec{v_j} = \lambda_j \cdot \vec{v_j} , 
$$
$$
\ j \in \{0, 1, 2\}, \lambda_i < \lambda_j\ \text{if}\ i\ <\ j,
$$
where $k$ is the number of neighbors considered in the neighborhood of $g$, $p_i = \{x, y, z\}$ is the position of the neighbor grid in the global coordinate frame, $\bar{p}$ is the 3D centroid of the neighbors, $\lambda_j$ is the $j$-th eigenvalue of the covariance matrix, and $\vec{v_j}$ is the $j$-th eigenvector. The surface normal $\vec{n}$ of grid $g$ is the eigenvector $\vec{v_0}$ with the smallest absolute value of eigenvalue $\lambda_0$. 

% And we use the viewpoint $V = \{0, 0, 1\}$ to orient normal $\vec{n}$ consistently towards the viewpoint, they need to satisfy the equation: 
% $$
% \vec{n} \cdot V > 0
% $$

% \he{And the problem of determining the normal to a grid cell can be reduced to an analysis of the eigenvectors and eigenvalues (or PCA – Principal Component Analysis) of a covariance matrix created from the nearest neighbors of the query grid cell. } 
% More specifically, for each grid cell $g_i$, we assume it's is a point $p_i = \{x, y, z\}$ which $x$, $y$ is the position of the cell in global coordinate frame, and $z$ is the height value. Then we can assemble the covariance matrix $c$ as follows: 


% This approximation greatly reduces the complexity of the calculation.


The purpose of the slope estimation is to get the shape of the terrain and avoid navigating on a steep surface. For excavator applications, the width between the tracks or wheels is a good indicator of the navigation stability on rough terrain. Usually, when the area of a rough region is less than half the width between the excavator's tracks, the excavator can navigate through it without any trouble. Specifically in our excavator setup, the width of our excavator track is $0.6\ m$, so we chose the grid resolution $d_{res} = 0.2\ m$ and search the nearest eight neighbors, which covers the necessary area.
% \tian{To our experience, the terrain slope of the track width ($0.6\ m$ in our robot) is a suitable width that can guide the robot to walk. 
% So we chose the grid resolution $d_{res} = 0.2m$ and use eight neighborhood search method which means the search area size equals the track width. }

%To our experience, the area size or grid resolution $d_{res}$ equals to half of the width of the track is reasonable. A grid area that is too small is meaningless for the passage of excavators. And the neighbors search parameter $k = 9$ is enough for our geometric information computation to cover at least the width of the track.


% {两个方面，一个是resolution, 一个是radius}
% {resolution 取决于履带宽度？ 因为太小的grid cell对于挖掘机的通行是没有意义的，那么得知道多大的地形障碍(石头等)对挖掘机是有影响的(半个履带大小?)}
% {选择radius为8临域能够保证step height起码积攒3个履带宽度? slope反映履带宽度大小的平面的斜率？ 或者我们不讨论8临域的合理性。}
% {宽度大的影响   step height: 导致step height越大  slope: 不能反映真实斜率}
% {宽度小的影响   step height: 太小，不能反映陡坡  slope: 更准确} better 

\noindent\textbf{Step Height Estimation:}
The step height $h$ is computed as the largest height difference between the center point $p$ of the grid and its $k'$ nearest neighbors: 
% \he{still a gap between g and p, should we use g instead}
$$
h = \max{ (\text{abs}(p^z - p_i^z))}, i \in [1,k']
$$
Since slope is a description of variation in the terrain in a relatively small region, we choose to use a neighbor search parameter $k' = 7*7 > k$ that spans $1.4\ m$ to measure height change in a larger scope. For excavator applications, the step height calculation guarantees that the track does not traverse areas with extreme height differences. 

% \tian{The neighbors search parameter $k' = 7*7 > k$.  Because we store the average height in the grid, and we use step height to analyze whether slope will last for 3 grids, so the range should be $7$ (For the center grid, there are 3 grids on each side). }
% We use step height in a bigger range to capture a large features -- at least 0.6 m -- the width of the track

% \tian{Add explanation here!!!}
% \tian{can we use roughness as a decay? If too rough, then step height is a better measurement; otherwise, step height is a better measurement.}
% \tian{Fix neighbor issue}
% The slope of the terrain is a local description of the terrain, which might be sensitive to noise. 

% \noindent\textbf{Roughness Estimation:}
% % The terrain roughness $r$ is calculated as the standard deviation of the terrain height values to the fitting plane. The distance $d$ from the center point $p$ of the grid to the fitting plane of $k$ neighboring girds, is calculated as:
% % $$
% % d = \frac{\vec{p\bar{p}} \cdot \vec{n}}{| \vec{n} |}
% % $$
% % where $\vec{n}$ is the surface normal vector of the fitting plane and $\bar{p}$ is a point in the plane.
% % Finally, the roughness estimation of the grid $g$ can be computed as:
% % $$
% % r = \sqrt{ \sum_{i=1}^{k} (d_i)^2 }
% % $$
% \he{I thought we don't need roughness at all. Because excavators often work on uneven ground, the important thing is not the roughness but the material (soil, stone) This can be a good point}

\noindent\textbf{Geometric Traversability Estimation:}
Based on information about slope and step height of the terrain, we can calculate a geometric traversability score $T_{geo}$. According to the physical constraints of the robot, we create some critical values $s_{cri}$, $s_{safe}$, $h_{cri}$, $h_{safe}$,  as the thresholds for safety and danger detection. The purpose of those threshold values is to avoid danger when the surface condition exceeds the limits of the robot and to avoid more calculations when the surface is very flat. 
The formula for geometric traversability $T_{geo}$ for each grid is:

% The calculation of geometric traversability is determined based on the characteristics of the robot itself. 
% The track brings excellent terrain adaptability to the excavating robot. Therefore, the roughness of the terrain will not have a significant impact on the driving of the robot. 
% But the slope and step height are critical factors in determining the robot's traversability because of the high center of gravity.

% % \he{Give the specific value of the 490 document}
% In Fig. \ref{placeholder}, we can see that the slope is suitable for detecting dangerous areas such as pits or bumps. But we also notice some small areas(few numbers of cells) with high slopes on the map, usually caused by stones or pits on the ground. These areas should not be considered geometrically untraversable because they are too small to influence the robot. At this time, we need to use step height, which can be regarded as the integral of the slope, to judge those areas. So when the slope is large, but the step height is small, it should be treat as traversable. 
\vspace{-10pt}
\begin{equation}
\resizebox{.99 \hsize }{!}{$
T_{geo} = 
\begin{cases}
0& s > s_{cri} \ \text{or} \ h > h_{cri}\\
1& s < s_{safe} \ \text{and} \ h < h_{safe}\\
\max( 1 - (\alpha_1 \frac{s}{s_{cri}} + \alpha_2 \frac{h}{h_{cri}}) , 0 ) & \text{otherwise}
\end{cases},
$} \nonumber
\end{equation}
where the weights $\alpha_1$ and $\alpha_2$ sum up to 1. 
% In our case, we use 0.5 and 0.5, respectively.

% \he{Unlike the method describe \cite{geo1}, we don't calculate roughness score in $T_{geo}$ but keep slope and step height. Because in our usage, the excavator robot often work on uneven ground and can handle rough terrain most of the cases, while it is more sensitive and easy to fail when the slope or step height is very large. The important thing is not the roughness but the material, which accomplish by semantic information.}

% Unlike the method described in~\cite{geo1}, we exclude the use of a roughness score in $T_{geo}$. In our context, the excavator is more sensitive and prone to failure under extreme slopes and step heights, while it can usually handle uneven ground and relatively rough terrain. We also discover that the roughness measurement is not effective in the traversability computation. 
% For more detailed comparisons, please refer to the full report~\cite{guan2021ttm}. 
% For more detailed comparisons, please refer to the supplemental material. 

% In addition, the measurement of terrain roughness is accomplished through visual cues and texture information, as bumpy regions are classified from 2D semantic information, and this method produces a more meaningful output than geometric measurement.

% Because the value of RTK on the Z-axis is unstable, the value of Z may vary significantly at different times, so we save update time in the grid and only use the grid within a certain range $\triangle t$ at the current time for geometric information calculation. 

%We use slope and step height as major factors which contribute to dangerous non-traversable terrain, and use roughness only as a minor contributing factor towards $T_{geo}$, because slope and step height largely contribute to the navigability of the terrain. In addition, excavators can handle rough terrain most of the cases, while they are more sensitive and easy to fail when the slope or step height is very large.

% Explain formula to calculate those scores, and explain and justify our threshold
% explain hard negative and soft score??
% explain that we use both sensor

% parameters:
% 1. slope
% 2. resolution? / neighbors/radius
% 3. according to the height of the wheel

% step height as complementary to slope!! -- give absolute value
% roughness is not as important -- just contribute to danger value

% \noindent\textbf{Safe and Critical Threshold:}

% We use the specifications of our excavator to determine the safe and critical values. We use an XCMG XE490D excavator, which has a maximum climbing angle of 35 degrees. We use the typical recommended climbing angles for any vehicle as a safe climbing angle, which is 10 degrees. As a result, we set $s_{cri} = 30\ deg$ and $s_{safe} = 10\ deg$.

% For step height, we make sure that $h_{cri}$ and $h_{safe}$ comply with slope $s_{cri}$ and $s_{safe}$. We get an approximation of the maximum height allowed by $s_{cri}$ and $s_{safe}$, expanding three times the resolution $d_{res}$ along the surface:
% \begin{align*}
% h_{cri} &= 3\ tan(s_{cri}) \times d_{res} = 0.35\ m\\
% h_{safe} &= 3\ tan(s_{safe}) \times d_{res} = 0.10\ m
% \end{align*}


The step height estimation is complementary to slope estimation; it provides a global perspective, whereas slope is local terrain information. Combining these two specifications can help us remove noise in the map, such as bumps caused by dust, and ensure the robustness of the $T_{geo}$.

% For roughness, $r_{cri}$ is set to a heuristic value of $0.1\ m$ according to our experience that our robot can walk through steps less than $10\ cm$ high.




% \he{The result is not scale to 0~1!!!}
% roughness serve a a complimentary 

% \he{why we not use step height as the direct traversability but slope? noise? step height is the possible max influence of slope but can have some noise such as a pit and bump together?}
% \he{Only height values which were detected within a certain range $\delta f$ of frame numbers are considered in the traversability estimation process}


% \subsection{Traversability Estimation Combining Geometric and Semantic Information}
\subsection{Traversability with Geometric and Semantic Fusion}
\label{trav_est}

In this section, we describe our algorithm for geometric-semantic fusion. From the semantic and geometric information, we use a continuous traversability score $T\in [0, 1]$ to measure how easily the surface can be navigated. This is especially relevant to off-road scenarios because we prefer flat regions over bumpy roads to save energy. Moreover, when an excavator is navigating on a construction site, being able to correctly identify different regions is critical to avoid hazardous situations like flipping over.

The overall traversability score $T$ is calculated based on semantic terrain classes $C_{sem}$ and geometric traversability $T_{geo}$ on each grid:

% \begin{equation}
% \resizebox{.91 \hsize }{!}{$
% T = 
% \begin{cases}
% % 0& T_{sem} = 0 \ \text{or} \ T_{geo} = 0\\
% \alpha_{sem}\times T_{sem} + (1 - \alpha_{sem}) \times T_{geo} & T_{sem}\  exists\\
% (1-  \alpha_{penalty})\times T_{geo} + \alpha_{penalty} & \text{otherwise}
% \end{cases},
% $}
% \end{equation}
\vspace{-10pt}
\begin{equation}
\resizebox{.89 \hsize }{!}{$
T = 
\begin{cases}
0 & C_{sem} = \text{\{rock, excavator, obstacle, water\}}\\
1 & C_{sem} = \text{\{flat\}}\ \text{and}\ T_{geo} > 0\\
T_{geo} & \text{otherwise}\\
% T_{geo} & C_{sem} = \text{\{bumpy, mixture, unassigned\}}\\
% T_{geo} & \text{otherwise}
\end{cases},
$} \nonumber
\end{equation}

% \noindent where $\alpha_{sem}$ is the weight for semantic calculation and $\alpha_{penalty}$ is the penalty score without semantic information. In our case, we choose $\alpha_{sem} = 0.7$ and $\alpha_{penalty} = \tian{xx}$.


% \he{Based on our formulation, 
% we first make sure that if the terrain is considered non-traversable in either geometric calculation or semantic inference, the overall traversability is 0. 
% We want to make sure the robot should absolutely avoid dangerous regions from either geometric or semantic perspective. 
% Then, we use semantic information ${flat}$ to correct the possible noise in $T_{geo}$. 
% In other situations (\{bumpy, water, mixed\}), we choose to trust the geometric information. }

% we use a weighted sum of those two terms for the traversability estimation. It is possible that there is only geometric information, since LiDAR has a wider view than the RGB camera; in this case, we choose to add a penalty of 0.3 to the traversability due to lack of information.

% Based on our formulation, we make sure that the robot avoids any obstacles like rocks or excavators and forbidden regions like water. 
% We also consider flat regions as traversable regions with a score of 1. In other cases like bumpy, mixed, or unassigned regions, we set the score according to the geometric information.
This method is simple yet more effective than other comparably complicated fusion methods~\cite{3d_cam_cmp3, semantic_for_planning_cmp2}, as demonstrated in Section~\ref{evaluation} and Section~\ref{aes_imp}.

% With our current scheme, we manage to minimize the use of continuous values in the final traversability map to reduce the number of grey regions to adapt to the effectiveness of existing planners.



% \subsection{Planning Based on TTM}
% \label{navi}

% We start with a novel post-processing step on the traversability map for planning. We remove some small non-traversable regions that satisfy all of the following criteria:
% \begin{itemize}
%     \item The region has an average traversability value less than some occupied threshold $t_{occ}$.
%     \item The region has a height less than the critical threshold of step height $h_{cri}$.
%     \item The spans of the region along the x-axis and the y-axis are less than half the distance between two tracks of the excavator $d_{track}$.
% \end{itemize}
% % traversability value less than \tian{xx}, maximum spanning less than 
% % half of the distance between two tracks of the excavator and height lower than critical threshold of step height $h_{cri}$.

% % that is less than half of the distance between two tracks of the excavator and is lower than the critical threshold of step height $h_{sci}$. 
% This post-processing step is mostly to accommodate existing planners, since they do not work well and fail to plan a feasible trajectory with too many scattered, noisy regions. After post-processing, we transform the traversability gridmap to a 2D occupancy gridmap as an input for path planning. We use the Hybrid A* planner~\cite{hybridA} to generate a path and send the trajectory to the motion controller, which guides the excavator to follow this trajectory. Some planning results can be found in~\ref{planner_vis}.


% In this step, the traversability map would be used for global path planner and guide robot navigation. 
% We first transform the 3D traversability Map to a 2D occupancy gridmap. Then  motion planners such as a Hybrid A*~\cite{hybridA} planner takes 2D gridamp as input and generates a path. There are two problems using 2D occupancy gridmap directly. First, because the robot working environment is rough and $T \neq 0$ in many grids, this will cause the planner to tend to bypass these rough areas and generate a tortuous path. Secondly, the tiny obstacles which can be completely ignored by excavator could lead to generate a bypassing trajectory.

% To tackle these problems, we use a threshold of $0.99$ to binarize the 2D occupancy gridmap so that our planner can ignore the obstacles ($T = 1$) that size less than track width ($60cm$). \comm{how about human...}
% Through the above operations, the planner can generate a path without unnecessary turns, while still avoiding dangerous obstacles. After the path is generated, the excavator motion controller is used to follow this trajectory to navigate.

% \comm{Should we have some picture here.}
% \comm{Should we claim global and local path planner?}

% traversability map ---> occ map ---> remove small block ---> planning ---> controller ----> move

% Based on the resulting occupancy gridmap, we show some planning results using Hybrid A*~\cite{hybridA} in Figure~\ref{fig:planner}. The implementation is based on publicly released code.

% \subsection{Mapping with Traversability Information}
% \label{mapping}
% % explain the localization and mapping part.

% Finally, we put together all the traversability information across frames for a global map. 


==> sections/4.5-ttm_planning.tex <==
\section{TTM-based Planning and Navigation}





We deploy our approach \ours{} on an excavator as part of the Autonomous Excavator System~\cite{Zhangeabc3164}. The AES system has a pipeline of perception, planning, and navigation modules. We integrate and evaluate our method through planning results and real-world navigation performance by using our mapping output, as shown in Figure~\ref{fig:aes}. Note that previous AES systems mainly focus on digging tasks, while our method focuses on providing accurate mapping estimation for navigation in unstructured environments.


\noindent\textbf{Post-processing after TTM:} We have a post-processing step on the traversability map before planning. We remove some non-traversable regions that satisfy all of the following criteria:
\vspace{-7pt}
\begin{itemize}
%   \setlength\itemsep{-0.3em}
    \item The region has a traversability value less than some occupied threshold $t_{occ}$.
    \item The spans of the region along the x-axis and the y-axis satisfy both: 1) less than half the distance between two tracks of the excavator $d_{track}$ and 2) an average height less than the height $h_{cab}$, which is the distance from the bottom of the cabin to the ground.
\end{itemize}
\vspace{-7pt}
% traversability value less than \tian{xx}, maximum spanning less than 
% half of the distance between two tracks of the excavator and height lower than critical threshold of step height $h_{cri}$.

% that is less than half of the distance between two tracks of the excavator and is lower than the critical threshold of step height $h_{sci}$. 

% After post-processing, we transform the traversability gridmap to a 2D occupancy gridmap as an input for path planning. We use the Hybrid A* planner~\cite{hybridA} to generate a path and send the trajectory to the motion controller, which guides the excavator to follow this trajectory. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OPTION 1 start
This post-processing step is mostly to accommodate existing planners, since they do not work well and fail to plan a feasible trajectory with too many scattered, noisy regions. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OPTION 1 end

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OPTION 2 start

\noindent\textbf{TTM-Based Planning:} We use Hybrid A*~\cite{hybridA} to calculate a trajectory based on the traversability map output from \ours{} after post-processing step. Hybrid A* is a global path planner based on a 2D occupancy girdmap as an input for path planning. The planner will generate a path and send the trajectory motion controllers, which guide the excavator to follow this trajectory.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OPTION 2 end












\noindent We briefly explain other components in AES framework:
% \vspace{-7pt}
\begin{itemize}
%   \setlength\itemsep{-0.3em}
    % \item \textbf{Trajectory Planner:} We use Hybrid A*~\cite{hybridA} to calculate a trajectory based on the traversability map output from \ours{}.
    \item \textbf{Tracking Controller:} This module can adjust the steering of the robot for path following.
    \item \textbf{Speed Controller:} This module can adjust the speed of the robot.
\end{itemize}
\vspace{-7pt}
%Please refer to AES~\cite{Zhangeabc3164} for more details. 
More results based on \ours{}-integrated planner and its benefits are given in Section~\ref{aes_imp}.

% In this step, the traversability map would be used for global path planner and guide robot navigation. 
% We first transform the 3D traversability Map to a 2D occupancy gridmap. Then  motion planners such as a Hybrid A*~\cite{hybridA} planner takes 2D gridamp as input and generates a path. There are two problems using 2D occupancy gridmap directly. First, because the robot working environment is rough and $T \neq 0$ in many grids, this will cause the planner to tend to bypass these rough areas and generate a tortuous path. Secondly, the tiny obstacles which can be completely ignored by excavator could lead to generate a bypassing trajectory.

% To tackle these problems, we use a threshold of $0.99$ to binarize the 2D occupancy gridmap so that our planner can ignore the obstacles ($T = 1$) that size less than track width ($60cm$). \comm{how about human...}
% Through the above operations, the planner can generate a path without unnecessary turns, while still avoiding dangerous obstacles. After the path is generated, the excavator motion controller is used to follow this trajectory to navigate.

% \comm{Should we have some picture here.}
% \comm{Should we claim global and local path planner?}

% traversability map ---> occ map ---> remove small block ---> planning ---> controller ----> move

% Based on the resulting occupancy gridmap, we show some planning results using Hybrid A*~\cite{hybridA} in Figure~\ref{fig:planner}. The implementation is based on publicly released code.


% Finally, we put together all the traversability information across frames for a global map. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/aes3.png}
    \caption{\textbf{\ours{}-based planning for autonomous excavation:} We show the components of AES as {blue} blocks and highlight our method \ours{} using a {red} block. We use green blocks to represent the TTM-based trajectory computation module.}
    \label{fig:aes}
    \vspace{-15pt}
    % \vspace{-18pt}
\end{figure}

